A Survey on Intrinsic Images: Delving Deep Into Lambert and Beyond

Intrinsic imaging or intrinsic image decomposition has traditionally been described as the problem of decomposing an image into two layers: a reflectance, the albedo invariant color of the material; and a shading, produced by the interaction between light and geometry. Deep learning techniques have been broadly applied in recent years to increase the accuracy of those separations. In this survey, we overview those results in context of well-known intrinsic image data sets and relevant metrics used in the literature, discussing their suitability to predict a desirable intrinsic image decomposition. Although the Lambertian assumption is still a foundational basis for many methods, we show that there is increasing awareness on the potential of more sophisticated physically-principled components of the image formation process, that is, optically accurate material models and geometry, and more complete inverse light transport estimations. We classify these methods in terms of the type of decomposition, considering the priors and models used, as well as the learning architecture and methodology driving the decomposition process. We also provide insights about future directions for research, given the recent advances in neural, inverse and differentiable rendering techniques.

==> sec/definition.tex <==

\section{Overview}
\label{sec:intro}


The appearance of an object in the physical world is determined by the complex interaction between the light, the material, and the geometry of the scene that contains it. Capturing this information in isolation for post-processing operations such as relighting o re-texturing can be done with different setups. 
The illumination is most frequently obtained by taking a light probe, which is 360º HDR picture of the environment.
%~\cite{Debevec:1998,Debevec:2000,Ramamoorthi:2001}. 
%For instance, this set up has been used to estimate positions of multiple light sources in a scene~\cite{Zhang:2001,Hougen1993}. 
The material properties can be captured with different devices. Among such devices, the \textit{goniophotometer} is the most accurate one to obtain the radiance under all possible combinations of incoming and outgoing light and view directions, capturing the behavior of the material in the form of Bidirectional Texture Functions.
%~\cite{muller2004,Filip2009,Nam2016}. 
% The most accurate representation of a material is given by the Bidirectional Texture Function or BRDFs~\cite{muller2004,Filip2009,Nam2016}, which encode tabulated the behavior of a material under all possible combinations of incoming and outgoing light and view directions. 
Finally, geometry can be obtained accurately with stereo cameras or depth sensors. 
%
These setups, however, require the use of specific devices and planning, and are not useful for on-the-wild situations where the only available device at hand is a conventional photographic camera.
% information we have from the scene is a single image.



When a light photon hits a pixel of the camera sensor, it integrates all the information that conforms the scene --geometry, materials and illumination-- in a single value, making the problem of recovering back this data an ill-posed one. 
%although critical for many computational photography applications, 
%is highly ill-posed.
%The most common way to capture appearance is by means of 
%Appearance is usually captured with more conventional methods such as 
%an image, in which case, all the information that convey the scene is integrated into the pixels of the camera sensor. 
%
A typical strategy to obtain this latent information involves 
%to recover this data is by 
fitting an analytical function parameterized by geometry, light and material, problem which is
%When all the components are parameterized in a function, the problem is 
known as \textit{inverse rendering}. This estimated model will allow to fully modify and \textit{re-render} the scene in post-processing, e.g. changing the illumination or viewpoint. The complexity of such model will determine the degree of realism of the matched scene, along with the difficulty in estimating its parameters, and the editing capabilities.

% that will allow to \textit{re-render} the scene e.g. with different illuminations or viewpoints, this problem is known as inverse rendering, and  A flexible model that includes all the components and allows to fully recreae, and \textit{re-render} the scene, is usually very hard to fit, in this case, the problem is known as inverse rendering.


The intrinsic images model firstly introduced by Barrow and Tenenbaum~\cite{Barrow1972}, is a simple yet accurate way for inversely modeling the appearance of a scene without the need to explicitly define the geometry or the illumination. Instead, it states that 
%t models the input scene as the pixel-wise multiplication of two components: one image that represent the materials, and one image that represents the illumination, 
an image $\mathbf{I}$ captured with a conventional photographic camera can be represented as the pixel-wise multiplication of two images, as shown in Figure~\ref{fig:introintrinsicexample}-b,
 
%
\begin{equation}\label{eq:introintrinsic}
\mathbf{I}_c(x) = \mathbf{R}_c(x) \times \mathbf{S}_c(x)
%{I_c(x)} = {R_c(x)} \times {S_c(x)}
\end{equation}
%
where $x$ is a pixel in the image, and $\text{c} \in \{\text{R},\text{G},\text{B}\}$ is the color channel or spectral band. The reflectance $\mathbf{R}$, or albedo, layer describes the diffuse color of the material and is invariant to illumination. The illumination layer $\mathbf{S}$ contains information about shading and shadows, and integrates the interaction between geometry and incoming light, usually containing also inter-reflections. 

In order to be physically accurate, this decomposition requires that the materials that compound the scene present Lambertian or diffuse reflection. That is, the reflected light (more technically, the surface luminance intensity) will be the same regardless of the observer's position, only obeying Lambert's cosine law. A huge number of materials in the real-world follow this property such as matte wall painting, unpolished wood, or freshly fallen snow. However, Lambertian reflections from polished surfaces are frequently accompanied by a specular or glossy reflection. The effect is maximally observed at the perfect reflection angle and falls off sharply. Several analytic models account for this effect such as Phong or Cook-Torrance. In the context of intrinsic decomposition, the specular highlights are usually accounted for as part of the shading layer, or less frequently, as an extra layer which is added to the initial ones, thus increasing the number of unknowns in the system.
 
Obtaining these components from a single image is a major challenge as for each known value of the input image there are two unknowns, therefore, infinite number of combinations that can satisfy Equation~\ref{eq:introintrinsic} (e.g.  Figure~\ref{fig:introintrinsicexample}-d). To make the problem tractable, existing methods impose additional constraints or make certain assumptions about the components. In the following, the most common approaches are reviewed. 




\begin{figure}[htb]
	\centering
	\includegraphics[width=0.95\textwidth]{example_and_edits.pdf}
	\caption{Intrinsic decomposition ambiguity (a)-(c) (inspired by \protect\cite{Bonneel2017}), and example of editing (d). (a) Input image $\protect \mathbf{I}$. (b) Decomposition into reflectance $\protect \mathbf{R}$ (top) and shading image $\protect \mathbf{S}$ (bottom). (c) Example of ambiguity in the decomposition, the product of these two images also yields the same input image $\protect \mathbf{I}$. (d) Editing example: both layers have been modified separately and combined to alter the appearance of the input image. }
	\label{fig:introintrinsicexample}	
	%\vspace{-5mm}
\end{figure}



\section{Priors and Methods to Constrain the Problem}

Priors and constraints are some statistical tools and methods which are used to encode existing beliefs about a problem. In the intrinsic decomposition problem, several priors have been developed to help disambiguate the decomposition along with several assumptions and ad hoc user interfaces. 
From a general perspective, the type of constraints can be classified into: local constraints, such as those which operate at local neighborhoods around image pixels; global constraints, which extend the notion of neighborhood to any pixel in the image; and priors about the distribution of the values of each component --the shading, the reflectance, or the illumination. 
%
Besides, another type of classification can be done by analyzing the source of the knowledge which originated such constraints. This information might come: automatically from existing theories of the human vision and texture perception, defined by the user,
%, such as user strokes which help incorporate prior knowledge of the human perception; 
or directly learned from the data. In the following, the latter classification  is developed in detail (see the state-of-the-art report of Bonneel et al.~\cite{Bonneel2017} for a more thorough evaluation with examples).
%
%, which are derived from the data itself. In the following, we develop the later 



\subsection*{Automatic Priors}

There exist a number of automatic priors that affect different aspects of the decomposition:

%\paragraph*{Prior from human vision and }
%\subsection{Retinex} 
\textbf{Shading} The initial techniques that addressed the intrinsic decomposition problem relied on theories of the human vision which relate local changes of intensity with either changes in reflectance or shading. 
The main theory was Retinex, 
%developed by Land and McCann~\cite{Land71}, 
which stated that the perceived color of an object remains constant as long as the reflectance ratios do not change, even if the light color changes. 
Inspired by it, 
%developed the Retinex theory to account for the perception of color in human vision. 
%The Retinex theory was developed by Land and McCann~\cite{Land71} to account for the perception of color in human vision.
%They came out with the color constancy theory which states that the perceived color of an object remains constant as long as the reflectance ratios do not change. This theory holds even if the light color changes. 
% Edge is either a reflectance or illumination change
%Later on, 
Horn~\cite{Horn74} implemented this theory in 2D images and presented a method to obtain the decomposition from black and white images assuming that sharp reflectance changes cause intensity discontinuities, while shading is a smooth function.
% Changes in reflectance are associated with changes in chromaticity
These types of constraints were implemented by thresholding local pixel derivatives to distinguish a change in reflectance from a change in shading. 
% \cite{tappen2005recovering}. 

\textbf{Reflectance} 
The extension of Horn's work to colored images was done by Funt el al.~\cite{Funt92recoveringshading} who associated changes in reflectance with local changes in chromaticity, and enforced integrability of the shading at these points like previous methods did.
%enforced integrability of the shading at these detected gradients. 
Propagating the shading values to their neighboring pixels was done by diffusion, solving the subsequent Poisson equation with a Fourier transformation. 
Later, several works extended this idea globally by assuming that the amount of different reflectances is sparse and performing color clustering within close-form or probabilistic frameworks \cite{garces2012intrinsic,Bell2014}. %Gehler2011

\textbf{Texture} Textured areas provide a very strong cue about regions of the image which should have the same reflectance values.
% regardless of how they are illuminated. 
The challenge here lies in finding texture descriptors and similarity metrics among them which are invariant to changes in illumination and geometry. In an optimization framework, these constraints are imposed over both local and non-local areas of the image~\cite{zhao2012closed}.


\textbf{Lighting} The type of light that illuminates the scene is critical for its appearance. In general, most of the methods assume that the images are white-balanced, and illuminated by a single light source. This can be further constrained assuming that the scene is illuminated by a narrow-band sensor such as Planckian light or Daylight. In that case, the reflectance of a single object forms a line in log-chromaticity space. This has been implemented following the color lines model~\cite{Omer2004} or entropy minimization~\cite{Fin04intrinsic}.




\subsection*{User Defined Constraints}

Another set of techniques rely on automatic priors \textit{and} user intervention. The first method to incorporate this kind of input into an optimization framework was 
Bousseau et al.~\cite{bousseau2009user}. They assumed that local reflectance variations lie in a 2D plane in RGB space, not containing black, and introduced three types of strokes with different semantics: constant-reflectance, constant-illumination, and fixed-illumination. The result of this set of methods is pretty compelling, although creating the appropriate strokes for each image may be challenging for unskilled users.
%Their method produces very compelling results, although creating the appropriate strokes for each image may be challenging for unskilled users.


\subsection*{Learning from Data}

Finally, a well-known strategy to solve this problem consists of learning the constraints directly from the data. The first method using this kind of approach~\cite{tappen2005recovering} used machine learning to classify the derivatives of the image as produced either by illumination or albedo. Ten classifiers were trained with a set of computer-generated images containing only reflectance or illumination components. Due to the high ambiguity, single classifiers were not enough, and they required to combine them with probabilistic propagation methods such as Markov Random Fields.
As in many other fields in computer vision, deep learning methods have also marked a before and an after in the way this problem has been tackled. 
The leading strategies nowadays combine fully-supervised learning, using human-annotated and rendered datasets, with self-supervised learning, using multiple images of the same scene with varying illumination~\cite{li2018cgintrinsics}.




\section{Applications}
Having the intrinsic components is useful for any task that would require some knowledge about lighting or materials of the scene. For example, changing the materials of a scene is simplified to edit the reflectance layer; segmentation is improved if the reflectance layer is used instead of the original input image; or stylization and relighting can be done more accurately by optimizing the shading and reflectance components separately. An example of such edits is shown in Figure~\ref{fig:introintrinsicexample}-d.


\paragraph{\textbf{Cross-References}}
Retinex Theory, Rendering Natural Phenomena 

